Fairness and Diversity in Recommender Systems: A Survey

Recommender systems are effective tools for mitigating information overload and have seen extensive applications across various domains. However, the single focus on utility goals proves to be inadequate in addressing real-world concerns, leading to increasing attention to fairness-aware and diversity-aware recommender systems. While most existing studies explore fairness and diversity independently, we identify strong connections between these two domains. In this survey, we first discuss each of them individually and then dive into their connections. Additionally, motivated by the concepts of user-level and item-level fairness, we broaden the understanding of diversity to encompass not only the item level but also the user level. With this expanded perspective on user and item-level diversity, we re-interpret fairness studies from the viewpoint of diversity. This fresh perspective enhances our understanding of fairness-related work and paves the way for potential future research directions. Papers discussed in this survey along with public code links are available at https://github.com/YuyingZhao/Awesome-Fairness-and-Diversity-Papers-in-Recommender-Systems .

==> relatedwork.tex <==
\vspace{-1ex}
\section{Related Work}\label{sec-relatedwork}
%\td{I think this whole subsection can be removed since this is a very general direction, and also we only focus on a single task of node classification here with fixing the underlying encoder to be a GNN}
%\textbf{Node Representation Learning}
%Learning informative node representation is crucial in completing tasks such as node classification and link prediction. Based on how we regularize the similarity of representations between pairs of nodes, conventional node representation learning approaches can be summarized into two categorizes: factorization-based approaches~\cite{qiu2018network} where the similarity is regularized by some deterministic metric observed from graph topology and random walk-based approaches~\cite{perozzi2014deepwalk} where the similarity is regularized by stochastic measures given by random walks. GNNs have gained popularity in node representation learning, owing to the proximity-encoding power of propagation and learning power of linear transformation~\cite{GCN,GCNII, Graphsage}. This work also employs GNNs as encoder to obtain fair node representations.

%\noindent \textbf{Fairness on Graph Neural Networks}
Most prior work on GNNs exclusively focus on optimizing the model utility while totally ignoring the bias encoded in the learned node representations, which would unavoidably cause social risks in high-stake discriminatory decisions~\cite{EDITS}. 
%\td{Assuming people are reluctant to share sensitive features,} 
%In view that people are reluctant to share their sensitive features, 
FairGNN~\cite{dai2021say} leverages a sensitive feature estimator to enhance the amount of the sensitive attributes, 
which greatly benefits their adversarial debiasing procedure. NIFTY~\cite{nifty} proposes a novel triplet-based objective function and a layer-wise weight normalization using the Lipschitz constant to promote counterfactual fairness and stability of the resulted node representations. EDITS~\cite{EDITS} systematically summarizes the biased node representation learning into attribute bias and structure bias, and employs the Wasserstein distance approximator to alternately debias node features and network topology. More recently, REFEREE~\cite{REFEREE} was proposed to provide structural explanations of bias in GNNs. Different from previous work, we study a novel problem that feature propagation could cause correlation variation and sensitive leakage to innocuous features, and our proposed framework FairVGNN expects to learn which feature channels should be masked to alleviate discrimination considering the effect of correlation variation. Recently, others have also explored this concept of varying correlation during feature propagation towards developing deeper GNNs~\cite{DeCorr}. Besides the fairness issue by sensitive attributes, bias can also come from the node degree~\cite{tang2020investigating}, graph condensation\cite{jin2021graph}, or even class distribution~\cite{dpgnn}, which we leave for future investigations.





